Inverse vector-valued Sturm-Liouville problem. I. Uniqueness theorem

This paper starts a series devoted to the vector-valued Sturm-Liouville problem $-\psi''+V(x)\psi=\lambda\psi$, $\psi\in L^2([0,1];\mathbb{C}^N)$, with separated boundary conditions. The overall goal of the series is to give a complete characterization of classes of spectral data corresponding to potentials $V=V^*\in L^p([0,1];\mathbb{C}^{N\times N})$ for a fixed $1\le p <+\infty$ and separated boundary conditions having the most general form. In the first paper we briefly describe our approach to this inverse problem and prove some preliminary results including the relevant uniqueness theorem.

==> UTPackage.tex <==
\makeatletter
\def\ifemptyarg#1{%
  \if\relax\detokenize{#1}\relax % H. Oberdiek
    \expandafter \@firstoftwo
  \else
    \expandafter \@secondoftwo
  \fi}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter

\let\@Indchar=R

\newcommand{\Ind}[1][]{
  \ifemptyarg{#1}
    {\@Ind}
    {\@IndgammaDub[#1]}
}
\def\@Ind{\@ifnextchar+{\@Indp}{\@ifnextchar-{\@Indp}{\@Indnil}}
}
\def\@Indp#1{\@ifnextchar\perp{\@Indchar_#1^}{\@Indchar_#1}
  }

\def\@IndgammaDub[#1]{\@ifnextchar[{\@IndgammaDubb[#1]}{\@Indgamma[#1]}}

\def\@IndgammaDubb[#1][#2]{\@ifnextchar+{\@IndgammaDubp[#1][#2]}
   {\@ifnextchar-{\@IndgammaDubp[#1][#2]}{\@IndnilgammaDub[#1][#2]}}
  }
  
\def\@IndgammaDubp[#1][#2]#3{
  \@ifnextchar\perp{\@IndgammaDubpperp[#1][#2]#3}{
      \if\FirstChar[#1]- 
        \@Indchar_{#3}^{[-\gamma_{\EatFirstChar#1},#2]}
      \else \if\FirstChar[#1]\pm
          \@Indchar_{#3}^{[\pm\gamma_{\EatFirstChar#1},#2]}
          \else
          \@Indchar_{#3}^{[\gamma_{#1},#2]}\fi
      \fi}
}
\def\@IndgammaDubpperp[#1][#2]#3#4{
    \if\FirstChar[#1]- 
    {\@Indchar_{#3}^{[-\gamma_{\EatFirstChar#1},#2]}}^\perp
      \else \if\FirstChar[#1]\pm
        {\@Indchar_{#3}^{[\pm\gamma_{\EatFirstChar#1},#2]}}^\perp\
        \else
    {\@Indchar_{#3}^{[\gamma_{#1},#2]}}^\perp\fi\fi
}

\def\@IndnilgammaDub[#1][#2]{
  \@ifnextchar_{\@IndnillgammaDub[#1][#2]}{\@IndnilgammaperpDub[#1][#2]}
}
\def\@IndnilgammaperpDub[#1][#2]{
  \@ifnextchar\perp{
  \if\FirstChar[#1]-{\@Indchar^{[-\gamma_{\EatFirstChar#1},#2]}}^
        \else \if\FirstChar[#1]\pm
        {\@Indchar^{[\pm\gamma_{\EatFirstChar#1},#2]}}^
        \else {\@Indchar^{[\gamma_{#1},#2]}}^ \fi
    \fi
    }{\if\FirstChar[#1]-{{\@Indchar^{[-\gamma_{\EatFirstChar#1},#2]}}}
        \else \if\FirstChar[#1]\pm
     {{\@Indchar^{[\pm\gamma_{\EatFirstChar#1},#2]}}}
        \else {{\@Indchar^{[\gamma_{#1},#2]}}} \fi
    \fi}
}

%\if\FirstChar[#1]-
%
%  \else \if\FirstChar[#1]\pm
%
%    \else
%
%    \fi
%  \fi


\def\@IndnillgammaDub[#1][#2]_#3{
  \@ifnextchar\perp{
  \if\FirstChar[#1]-
  {\@Indchar^{[-\gamma_{\EatFirstChar#1},#2]}_{#3}}^
  \else \if\FirstChar[#1]\pm
  {\@Indchar^{[\pm\gamma_{\EatFirstChar#1},#2]}_{#3}}^
    \else
    {\@Indchar^{[\gamma_{#1},#2]}_{#3}}^
    \fi
  \fi
}{\if\FirstChar[#1]-
  \@Indchar_{#3}^{[-\gamma_{\EatFirstChar#1},#2]}
  \else \if\FirstChar[#1]\pm
    \@Indchar_{#3}^{[\pm\gamma_{\EatFirstChar#1},#2]}
    \else
      \@Indchar_{#3}^{[\gamma_{#1},#2]}
    \fi
  \fi
}}
%%%%%%%%%%%%%
\def\@Indgamma[#1]{\@ifnextchar+{\@Indgammap[#1]}
   {\@ifnextchar-{\@Indgammap[#1]}{\@Indnilgamma[#1]}}
  }
  
\def\@Indgammap[#1]#2{
  \@ifnextchar\perp{\@Indgammapperp[#1]#2}{\if\FirstChar[#1]-
    \@Indchar_{#2}^{[-\gamma_{\EatFirstChar#1}]}
  \else \if\FirstChar[#1]\pm
    \@Indchar_{#2}^{[\pm\gamma_{\EatFirstChar#1}]}
    \else
        \@Indchar_{#2}^{[\gamma_{#1}]}
    \fi
  \fi
  }
}
\def\@Indgammapperp[#1]#2#3{{\@Indchar_{#2}^{[\gamma_{#1}]}}^\perp}

\newcommand\@Indnil{
  \@ifnextchar_{\@Indnill}{\@Indnilperp}
}
\def\@Indnilperp{\@ifnextchar\perp{\@Indchar^}{\@Indchar}
  }
\def\@Indnill_#1{
  \@ifnextchar\perp{\@Indchar_{#1}^}{\@Indchar_{#1}}
}
\def\@Indnilgamma[#1]{
  \@ifnextchar_{\@Indnillgamma[#1]}{\@Indnilgammaperp[#1]}
}
\def\@Indnilgammaperp[#1]{
  \@ifnextchar\perp{\if\FirstChar[#1]-
    {\@Indchar^{[-\gamma_{\EatFirstChar#1}]}}^
  \else \if\FirstChar[#1]\pm
    {\@Indchar^{[\pm\gamma_{\EatFirstChar#1}]}}^
    \else
        {\@Indchar^{[\gamma_{#1}]}}^
    \fi
  \fi}{\if\FirstChar[#1]-
    \@Indchar^{[-\gamma_{\EatFirstChar#1}]}
  \else \if\FirstChar[#1]\pm
    \@Indchar^{[\pm\gamma_{\EatFirstChar#1}]}
    \else
        \@Indchar^{[\gamma_{#1}]}
    \fi
  \fi}
}
\def\@Indnillgamma[#1]_#2{
  \@ifnextchar\perp{\if\FirstChar[#1]-
    {\@Indchar_{#2}^{[-\gamma_{\EatFirstChar#1}]}}^
  \else \if\FirstChar[#1]\pm
    {\@Indchar_{#2}^{[\pm\gamma_{\EatFirstChar#1}]}}^
    \else
        {\@Indchar_{#2}^{[\gamma_{#1}]}}^
    \fi
  \fi}{\if\FirstChar[#1]-
    \@Indchar_{#2}^{[-\gamma_{\EatFirstChar#1}]}
  \else \if\FirstChar[#1]\pm
    \@Indchar_{#2}^{[\pm\gamma_{\EatFirstChar#1}]}
    \else
        \@Indchar_{#2}^{[\gamma_{#1}]}
    \fi
  \fi}
}

\renewcommand\b{\let\@Indchar=\mathfrak{b}\Ind}

\newcommand\Es{\let\@Indchar=E\Ind}

\renewcommand\P{\let\@Indchar=P\Ind}

\newcommand\eb{\let\@Indchar=e\Ind}

\newcommand\hb{\let\@Indchar=h\Ind}

\newcommand\ev{\let\@Indchar=\lambda\Ind}

\def\FirstChar[#1]{\@FirstChar#1.}

\def\@FirstChar#1#2.{#1}

\def\EatFirstChar#1{\relax}

\makeatother


